Enhancing Reward Models for High-quality Image Generation: Beyond Text-Image Alignment

Contemporary image generation systems have achieved high fidelity and superior aesthetic quality beyond basic text-image alignment. However, existing evaluation frameworks have failed to evolve in parallel. This study reveals that human preference reward models fine-tuned based on CLIP and BLIP architectures have inherent flaws: they inappropriately assign low scores to images with rich details and high aesthetic value, creating a significant discrepancy with actual human aesthetic preferences. To address this issue, we design a novel evaluation score, ICT (Image-Contained-Text) score, that achieves and surpasses the objectives of text-image alignment by assessing the degree to which images represent textual content. Building upon this foundation, we further train an HP (High-Preference) score model using solely the image modality to enhance image aesthetics and detail quality while maintaining text-image alignment. Experiments demonstrate that the proposed evaluation model improves scoring accuracy by over 10\% compared to existing methods, and achieves significant results in optimizing state-of-the-art text-to-image models. This research provides theoretical and empirical support for evolving image generation technology toward higher-order human aesthetic preferences. Code is available at https://github.com/BarretBa/ICTHP.

==> tabs/geneval1.tex <==
\begin{table*}[!t] 
\centering
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Quantitative Evaluation of Optimization Results Across Reward Models on GenEval Benchmark.}} 
\label{tab:geneval}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{lccccccc}
\toprule
\small\textbf{Model} &
\small{\bf Mean $\uparrow$ } &
\small{\bf Single$\uparrow$} &
\small{\bf Two$\uparrow$} &
\small{\bf Counting$\uparrow$} &
\small{\bf Colors$\uparrow$} &
\small{\bf Position$\uparrow$} &
\small{\bf Color Attribution$\uparrow$}\\
\midrule
\small % SD v2.1 & 0.50 & 0.98 & 0.51 & 0.44 & 0.85 & 0.07 & 0.17  \\
\small SDXL & 0.55 & 0.98 & 0.74 & 0.39 & 0.85 & 0.15 & 0.23  \\
\small % IF-XL & 0.61 & 0.97 & 0.74 & 0.66 & 0.81 & 0.13 & 0.35 \\
\small % PixArt-$\alpha$ & 0.48 & 0.98 & 0.50 & 0.44 & 0.80 & 0.08 & 0.07 \\
\small DALL-E 2 & 0.52 & 0.94 & 0.66 & 0.49 & 0.77 & 0.10 & 0.19  \\
\small DALL-E 3 & 0.67 & 0.96 & 0.87 & 0.47 & 0.83 & \textbf{0.43} & 0.45 \\
\small SD3 & 0.68 & 0.98 & 0.84 & 0.66 & 0.74 & \underline{0.40} & 0.43  \\
\midrule
\small SD3.5-Turbo & 0.69 &  0.99 & 0.87 & 0.69 & 0.80 & 0.25 & 0.55 \\
\cdashline{1-8}[1pt/1pt]
\small + Imagereward & 0.70  & 0.99& 0.87 & 0.68 & 0.80 & 0.28 &  0.59\\
\small + HPS\_v2 & 0.69 & 0.98 & 0.86 & 0.68 & 0.81 & 0.27 & 0.57 \\
\small + Pickscore & 0.66 & 0.99 &0.85 & 0.67& 0.74 & 0.24 & 0.48 \\
\rowcolor[HTML]{E6E6FA}
\small \textbf{+ ICT-HP (Ours)} & \textbf{0.70} & \textbf{0.99} & \textbf{0.88} & 0.68 & 0.79 & 0.28  & \textbf{0.58} \\
\midrule
\small + CLIP(crash) & 0.13 & 0.38 & 0.04 & 0.06 & 0.26 & 0.01 & 0.03 \\
\rowcolor[HTML]{E6E6FA}
\small \textbf{+ ICT (Ours)} & \textbf{0.71} & \underline{0.98} & \textbf{0.88} & \textbf{0.70} & \textbf{0.81} & \textbf{0.31} & \textbf{0.56} \\
\bottomrule
\end{tabular}
}
\vspace{-1em}
\end{table*}

==> tabs/ictacc1.tex <==
% TODO：加引用
\begin{table}[htbp]
    \centering
    \caption{Preference prediction accuracy on test sets of Pick-High and Pickapic\_v2.}
    \resizebox{\linewidth}{!}{\begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Average}} & \multicolumn{3}{c}{\textbf{Pairwise Comparison}} \\
        \cmidrule(l){3-5}
        & & \textbf{$I_2 > I_1$} & \textbf{$I_3 > I_2$} & \textbf{$I_3 > I_1$} \\
        \midrule
        Random & 50.00 & 50.00 & 50.00 & 50.00 \\
        ICT-groundtruth & 87.55 & 62.80 & 99.87 & 99.98 \\
        \midrule
        CLIP & 60.30 & 64.29 & 52.80 & 63.79 \\
        ITC  & 57.36 & 63.33 & 48.42 & 60.31 \\
        ITM  & 63.39 & 63.88 & 58.28 & 67.99 \\
        Aesthetic & 68.19 & 50.90 & 77.81 & 75.83 \\
        ImgReward & 63.81 & 64.58 & 58.02 & 68.84 \\
        HPSv2 & 72.88 & 66.98 & 71.63 & 80.04 \\
        PickScore & 79.04 & 74.80 & 75.37 & 86.94 \\
        \midrule
        \textbf{ICT} & 87.58 & 64.65 & 100 & 100 \\
        \textbf{HP} & 88.47 & 64.97 & 100 & 100 \\
        \rowcolor[HTML]{E6E6FA}
        \textbf{ICT-HP} & \textbf{88.84} & 66.42 & 100 & 100 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:reward-comparison}
\end{table}


==> tabs/jpgaes1.tex <==
\begin{table}
\centering
\caption{JPEG Compressibility and Aesthetic Scores on Parti-Prompts[x]}
\label{tab:jpeg-aesthetics}
\resizebox{\linewidth}{!}{\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \textbf{JPEG} & \textbf{Aesthetic}  \\
 & \textbf{Compressibility $\uparrow$} & \textbf{Score $\uparrow$} \\
\midrule
SD3.5 & 374.80 & 6.307 \\
FLUX-dev & 270.58 & 6.436 \\
\midrule
SD3.5-Turbo & 313.10 & 6.293 \\
\cdashline{2-3}
\vspace{1.0mm}
+ CLIP(crash) & 279.98 & 5.175 \\
\textbf{+ ICT (Ours)} & 321.39 & 6.285 \\
% + HPS & 331.47 & 6.330 \\
% + PickScore & 334.23 & 6.752 \\
\rowcolor[HTML]{ECFAEC}
\textbf{+ ICT-HP (Ours)} & 330.23 & 6.300 \\
\rowcolor[HTML]{E6F3FF}
\textbf{+ HP (Ours)} & \textbf{334.86} & \textbf{6.448} \\
\bottomrule
\end{tabular}
}
\end{table}



